Towards Marrying Files to Objects

To deal with the constant growth of unstructured data, vendors have deployed scalable, resilient, and cost effective object-based storage systems built on RESTful web services. However, many applications rely on richer file-system APIs and semantics, and cannot benefit from object stores. This leads to storage sprawl, as object stores are deployed alongside file systems and data is accessed and managed across both systems in an ad-hoc fashion. We believe there is a critical need for a transparent merger of objects and files, consolidating data into a single platform. Such a merger would extend the capabilities of both object and file stores while preserving existing semantics and interfaces. In this position paper, we examine the viability of unifying object stores and file systems, and the various design tradeoffs that exist. Then, using our own implementation of an object-based, POSIX-complete file system, we experimentally demonstrate several critical design considerations.

==> sections/dataflow.tex <==
\subsection{Data access}
\label{section:dataflow}

The optimal design for an object-based file system depends heavily on how users
plan to access the data.
%
\ITEM{File-system access only} implies that all data is ingested, manipulated,
and retrieved through a file-system interface.
%
In this case, object storage acts merely as a provider of raw bytes to a file
system.
%
Such usage of an object storage is justified because of its low cost and high
scalability.
%
%
\ITEM{Complete dual access} provides an ability to ingest and process the data
through both object and file-system interfaces.
%
E.g., a newly created file appears in the object storage as a fresh object and,
vice verse, a newly created object manifests itself as a file in the file
system.
%
Complete dual access allows users to freely select, switch between, and combine
data processing applications.
%
%
\ITEM{Partial dual access} is provided by the systems that integrate in their
design a limited ability to access the data through both interfaces.
%
In one setup the data may be ingested solely through the object interface
(e.g., images from the IOT devices), but consumed using the file-system
interface (e.g., POSIX-based pattern recognition software).
%
Furthermore, the file system might display only the objects that existed before
the file system creation, but not the ones that were added later.
%

%
In the following sections we illustrate how data access requirements impact the
design of ObjectFS.
%


==> sections/figure_file.tex <==

\begin{figure}[t]
  \includegraphics[width=\linewidth]{images/file.pdf}
  \caption{Representation of an object as a file}
  \label{figure:file}
\end{figure}


==> sections/figure_overview.tex <==
\begin{figure}[t]
  \includegraphics[width=\linewidth]{images/overview.pdf}

  \vspace{10pt}

  \caption{An overview of the ObjectFS architecture}
  \label{fig:overview}
\end{figure}

